ChartEditor: A Human-AI Paired Tool for Authoring Pictorial Charts

Pictorial charts are favored for their memorability and visual appeal, offering a more engaging alternative to basic charts. However, their creation can be complex and time-consuming due to the lack of native support in popular visualization tools like Tableau. While AI-generated content (AIGC) tools have lowered the barrier to creating pictorial charts, they often lack precise design control. To address this issue, we introduce ChartEditor, a human-AI paired tool that transforms basic charts into pictorial versions based on user intent. ChartEditor decomposes chart images into visual components and organizes them within a hierarchical tree. Based on this tree, users can express their intent in natural language, which is then translated into modifications to the hierarchy. In addition, users can directly interact with and modify specific chart components via an intuitive interface to achieve fine-grained design control. A user study demonstrates the effectiveness and usability of ChartEditor in simplifying the creation of pictorial charts.

==> useless/3-formative.tex <==
\section{Formative Study}
To guide the design of \sys, we conducted a formative study aimed at understanding the challenges users face when authoring pictorial charts using existing tools.
Our objectives were twofold: (1) to identify the needs and interaction difficulties of users with varying levels of design expertise, and (2) to explore whether popular design tools offer features that could be adapted to improve the user experience.
To achieve these objectives, we conducted semi-structured interviews with a diverse group of participants with different levels of design expertise.
The interviews allowed for flexibility in exploring specific difficulties, areas of improvement, and potential features that could be integrated into a future system.

\subsection{Participants and Procedure}

We recruited 6 participants, including four students with entry-level design backgrounds  (P1\textasciitilde P4) and two experienced UX designers (P5\textasciitilde P6). 
The entry-level users were university students from various disciplines who frequently needed to create visual content for presentations and reports.
The UX designers had extensive experience in creating visualizations and user interfaces.
Each interview lasted approximately 30 minutes and consisted of two main tasks:
% The interviews were conducted by two interviewers.


\begin{enumerate}
    \item \textbf{Task 1:} Participants were instructed to create a pictorial chart using Adobe Illustrator and shared the challenges they encountered during this process.
    % This task aimed to explore the challenges they encountered during the creation process using traditional methods. 
    Participants were also asked to provide feedback on their experience with the software and their prior design experience.
    \item \textbf{Task 2:} Participants were shown a video demonstrating the usage of using three popular pictorial chart authoring tools \cite{xiao2023spark,wu2023viz2viz, zhang2020dataquilt}.
    Following the video, they were asked to provide feedback on the tools’ interaction and functionality.
\end{enumerate}



\subsection{Data Collection and Analysis}
Two researchers independently reviewed the interview transcripts to extract key observations, ideas, and issues.
They focused on specific keywords, challenges, and inefficiencies in interactions.
These data were cooperatively organized using thematic analysis \cite{braun2006using} and visualized by affinity diagram.
The process involved the following steps:

\begin{enumerate}
    \item \textbf{Key Idea Extraction:} Each researcher reviewed the interview transcripts and extracted notable observations related to user experience, interaction difficulties, and usability issues.
    \item \textbf{Idea Organization:} The researchers grouped related observations into categories, such as usability issues, interaction challenges, and feature suggestions.
    \item \textbf{Labeling and Grouping:} Each group of related ideas was labeled based on its thematic content. For example, issues related to interface complexity were grouped under ``Usability Challenges.''
    \item \textbf{Pattern Identification:} Common patterns across participants were identified, particularly concerning difficulties encountered during the chart authoring process and the strengths of popular tools.
\end{enumerate}

\subsection{Findings and Design decisions}
Figure~\ref{fig:affinity} is an affinity diagram created to visualize the analysis of the key themes from the interviews.
The analysis revealed several key themes regarding user frustrations with existing tools for authoring pictorial charts. 

\begin{enumerate}
\item \textbf{Complexity and Learning Curve:} Entry-level users (P1--P4) found advanced software like Adobe Illustrator overwhelming due to its complexity and steep learning curve. They expressed that the time required to learn the software was disproportionate to their occasional need for creating pictorial charts.

\item \textbf{Usability and Interaction Issues:} Both entry-level users and UX designers reported difficulties with precise interactions. They found it challenging to manipulate small visual elements, leading to frustration and imprecise chart representations.

\item \textbf{Frustration with AI-Generated Content:} Participants who experimented with AI-powered tools like \textit{MidJourney} or \textit{DALL·E} expressed dissatisfaction with the outputs. The AI-generated pictorial charts often did not align with their data or visual expectations, and there was limited support for manual adjustments.


\item \textbf{Workflow Constraints:} Existing tools were overly dependent on original data and involved cumbersome, multi-step processes, which hindered users' efficiency and flexibility. Specifically, this rigidity made it difficult to make quick adjustments or iterate on designs, slowing down the pictorial chart creation process.
\end{enumerate}


\begin{figure*}
    \centering
    \includegraphics[width=1\linewidth]{figure/affinity diagram.pdf}
    \caption{Affinity diagram of thematic analysis.}
    \label{fig:affinity}

\end{figure*}

Based on these findings, we made the following design decisions to develop the pictorial chart authoring tool that is more accessible, user-friendly, and efficient for entry-level users:

\begin{enumerate}
    \item \textbf{Simplify the Interface and Workflow for Non-Professional Users:} Design an intuitive interface with a minimal learning curve, allowing users without advanced design skills to create pictorial charts easily.

    \item \textbf{Integrate User-Controlled AI Assistance:} Incorporate AI capabilities that generate high-quality pictorial elements aligned with the basic chart, while providing options for users to refine and adjust the outputs to mitigate dissatisfaction with AI-generated content.
    
    \item \textbf{Enhance Flexibility by Enabling Direct Manipulation of Visual Elements:} Reduce dependence on the original data by enabling users to directly manipulate chart elements and images. This will streamline the workflow, giving users more freedom to iterate and adjust visual components quickly, without the need for constant data references.
    
\end{enumerate}


 




==> useless/6-Evaluation.tex <==
\section{Evaluation}
% We conduct two user studies. 
% The first examines the assessment of the interaction process and the outcomes of entry-level users while utilizing \sys, while the other explores the opinion of professional UX designers regarding the system's design process. 
% Section 6.1 and 6.2 introduce the participants and procedure of user study 1 and 2 and user study 1's quantity result.
% The section 6.3 provides the interview analyzed themes results.
% The opportunity perceived in the collaboration between human beings and AI in the creation of pictorial charts is qualitative research conducted through thematic analysis.

We conducted two user studies to evaluate the effectiveness of \sys. 
The first study focused on the experiences and outcomes of entry-level users, while the second study sought feedback from professional UX designers on the system's design process. 
These participants were distinct from the group involved in the formative study.
In this section, we outline the participants, procedures, and results of both studies, as well as the themes identified in the interviews conducted. 
In Sections 6.1 and 6.2, we detail the participants and procedures of the first and second user studies, respectively. In addition, Section 6.3 presents the findings of a qualitative study on the perceived opportunities in collaborating with AI in creating pictorial charts through thematic analysis.


\subsection{User Study 1}

Through the school's mailing list, we recruited and screened out 18 participants with entry-level design experience after random sampling.
The participants range in age from 18 to 41, with diverse educational backgrounds and fields of study, and have a need to author data into charts: one administrative staff (S1), seven undergraduate students (S2\~S8), seven postgraduate students (S9\~S15)  and three assistant professors (S16\~18) participated in this study. 
Based on their answers on a five-point Likert scale (where 1 was strongly disagree and 5 was strongly agree), participants claimed that they were willing to employ AI-assisted tools for the making of charts (M = 3.94, SD = 0.87). Participants were asked to select a chart from the provided basic chart library and use \sys to generate a pictorial chart. 
Participants were required to be on-site. 
A brief tutorial was provided before the user study began. 
Participants were then randomly assigned to one of the three chart themes, ensuring an equal number of participants in each group.
During the using process, participants were asked to think aloud while using the \sys to create a pictorial chart from the chosen chart. 
After using the session, participants completed two questionnaires, the NASA Task Load Index~\cite{hart2006nasa} and the System Evaluation 5-point Scale. Finally, we conducted a semi-structured interview with the participants. 
During the user research, we captured the audio data of the participants' think-aloud sessions and semi-structured interviews. We then transformed the audio files into text scripts written in dialogue format using the {\em iflyrec} platform.


\subsubsection{\textbf{NASA—TLX Questionnaire Result}}

Figures~\ref{fig:NASA1} and \ref{fig:NASA2} shows the individual workload using the NASA-TLX questionnaire.
In the process of organizing the results of the questionnaire, we found that there are certain differences in task load data based on the background of the participants. 
So after the experiment, we added a question to the participants to confirm their identity. 10 participants identified themselves as researchers (such as doctoral students, research assistants, and assistant professors), while another 10 participants identified themselves as non-researchers (such as undergraduate students, master's students, and administrative staff). 
Therefore, we grouped the participants into Researcher and Non-Researcher. The overall workload is 8.65 by calculating the average of all individual workloads. 
Figure~\ref{fig:NASA1} shows box plots of six task-load values for all participants, researchers, and non-researchers, and pairwise t-tests were conducted to calculate their differences. 
Figure~\ref{fig:NASA2} shows the difference in workload values for the same task between the two groups. 
There is no significant difference between the two groups of participants in the total task load; However, there was a statistically significant difference between the two groups of participants in the Performance and Frustration tasks: researchers had lower performance ratings for \sys compared to non-researchers (p=0.036), and higher Frustration ratings (p=0.032).

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.6\linewidth]{figure/boxplot-0.ds5m1lzwg7m.pdf}
    \caption{Box plot results of NASA-TLX six task-load rating values and t-test results}
    \label{fig:NASA1}
\end{figure}


\begin{figure}[t!]
    \centering
    \includegraphics[width=0.6\linewidth]{figure/violin-group-0.d1t5h1mcg9n-1.jpg}
    \caption{Difference in workload values between the non-researcher group and the researcher group}
    \label{fig:NASA2}
\end{figure}

\begin{figure*}[t!] % H forces the figure to be placed exactly here
    \centering
\includegraphics[width=0.79\textwidth]{figure/6.1-gallery.pdf} \\ % First row
    \caption{Example pictorial charts created with \sys in User Study 1. (a) shows a line-semantic chart theme; (b) presents a line-area chart theme; (c) illustrates a bar-unit chart theme; (d) shows a bar-height chart theme; (e) shows a pie-area chart theme; (f) presents a pie-semantic and pie-unit chart theme.}
    \label{fig:gallery}


\end{figure*}

\subsubsection{\textbf{System Evaluation 5-point Scale}}

The evaluation of the system revealed generally positive feedback across all categories, with mean scores ranging from 3.78 to 4.28. 
The highest-rated three categories were the error correction and undo functions (M = 4.28, SD = 0.67), Chart Tree functions (M = 4.22, SD = 0.65), and Interactive Design of the System Efficiency (M = 4.22, SD = 0.65). 
In contrast, the system's layout was rated slightly lower (M = 3.78, SD = 1.00), with higher variability, suggesting mixed opinions on its intuitiveness. An ANOVA test (F = 0.758, p = 0.640) showed no significant differences between categories, indicating that participants rated all aspects of the system similarly high. Pairwise t-tests further supported this finding, as no category pair demonstrated statistically significant differences (p > 0.05). 

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.9\linewidth]{figure/questionnaire.pdf}
    \caption{System Evaluation 5-point Scale Rating Distribution and questions}
    \label{fig:enter-label}
\end{figure}

\subsubsection{\textbf{Pictorial Chart Gallery}}
We present the results generated by participants under various themes during the experiment. For each theme, we selected the visually most compelling outcome, as shown in Figure~\ref{fig:gallery}. In the top left corner of each row, the basic chart is displayed, with the first column showing the results of automatic generation. To highlight the versatility of our method, different recommended design patterns for each chart type are applied, indicated in the top right corner. The second column illustrates the outcomes of interactive generation, with the corresponding operation mode also noted, while the third column details the process.

In Figure~\ref{fig:gallery}(a), automatic generation uses a running figure to represent points on the line chart, with an Olympic-themed background. However, since the chart depicts the number of male and female athletes, the participant used the one-to-group editing mode to replace the stickers with category-appropriate icons, achieving a better fit.
Both Figures~\ref{fig:gallery}(b) and \ref{fig:gallery}(d) were automatically filled with generated images and later refined with minimal manual adjustments for aesthetic purposes.
In Figure~\ref{fig:gallery}(c), the automatically generated chart filled bars with plastic material. Since the categories correspond to different industries, the participant employed the one-to-one editing mode to replace each bar with a more contextually relevant icon, yielding a more accurate visual representation.
Figure~\ref{fig:gallery}(d) shows a pie chart where images representing land and ocean replace the original pie segments. Manual edits were applied to regenerate these images in different styles, further enhancing visual appeal.
Finally, in Figure \ref{fig:gallery}(e), fruit stickers were used to represent categories, with an additional modification filling each region with quantities of fruit, visually reflecting the proportions.wo ye

\subsection{User Study 2}

We invited three industry UX designers to participate in the study. First, we demonstrated the use of other similar pictorial chart authoring tools~\cite{xiao2023spark,wu2023viz2viz,zhang2020dataquilt}. Then, a 5-minute tutorial on the \sys was provided. Afterward, the participants were allowed to freely explore the interactions and chart generation process within the software. After 20 minutes of exploration, the participants were asked to engage in a semi-structured interview, comparing the system’s performance in terms of interaction, usability, and flexibility with other chart authoring tools, design software, and AI image generation tools. The interview was conducted by two researchers, recorded, and later transcribed into written scripts for analysis.


\subsection{Thematic Analysis}
This section provides an evaluation of the system based on feedback collected through semi-structured interviews with a diverse group of participants from both user study 1 (entry-level users) and user study 2 (UX designers). 
\sys is assessed across various aspects of user experience, with a focus on understanding its strengths and identifying potential areas for improvement. 
This evaluation draws on insights regarding how the system supports user needs, facilitates creative tasks, and balances between automation and user control.
The thematic analysis method~\cite{braun2006using} is employed to analyze the data collected from the semi-structured interviews and observation.
The data was analyzed using open coding in a deductive, bottom-up approach by two researchers. The authors chose thematic analysis as it is well-suited for identifying recurring themes in participants' behaviors and viewpoints, making it an ideal method for examining user challenges with \sys. The interviews were independently coded by the two researchers using Freeform. Following this, they collaborated to discuss and compare their annotations, reaching a consensus to merge their codes into a unified set.

\textbf{Theme 1: System Usability and Design Experience}
\begin{itemize}
    \item \textbf{Entry-Level Users: Ease of Use and Intuitiveness}  They found the system’s interface intuitive and easy to use, especially for basic tasks. They appreciated the icon-based layout, which made navigation straightforward. One user mentioned, ``The icons make the meanings clear at first glance''. The real-time preview feature was also praised for helping users adjust their designs efficiently.
    \item \textbf{UX Designers: Interface Simplicity vs Advanced Needs}  They acknowledged the simplicity of the interface but highlighted the need for more design flexibility. They noted that while the system works well for basic tasks, it could offer more options for advanced users. Designers also suggested that the real-time preview feature, though valuable, could be improved to offer more detailed insights into design changes.
\end{itemize}

\textbf{Theme 2: Flexibility and Customization Options}
\begin{itemize}
    \item \textbf{Entry-Level Users: Basic Customization for Efficiency}  They felt that the system provided sufficient customization tools for their needs. The balance between simplicity and customization was seen as a strong point, and participants appreciated not being overwhelmed by too many options. One user commented, ``This element is too small to edit, but I can do it just by clicking the node corresponding to the tree''.
    \item \textbf{UX Designers: Advanced Customization for Complex Tasks}  They, on the other hand, expressed a need for more advanced customization options. They felt that while the system met basic needs, it could expand its offerings to cater to more complex design tasks. One designer suggested, ``It would be nice to have a few more custom options'', indicating room for growth in this area.
\end{itemize}

\textbf{Theme 3: AI-Driven Assistance and Automation}
\begin{itemize}
    \item \textbf{Entry-Level Users: AI-Powered Time-Saving Tools} They praised the AI features for speeding up routine tasks, such as generating icons and visual elements. They appreciated how the AI could handle vague design inputs and transform them into usable outputs. One user mentioned, ``The AI function helps a lot'', especially for those who weren’t confident in their design skills.
    \item \textbf{UX Designers: AI Performance and Precision for Professional Use}  They acknowledged the potential of AI-driven features but noted that the system’s automation sometimes lacked refinement. They pointed out that while the AI was useful for generating ideas, it often required manual adjustments to meet professional standards. They suggested improvements in how the AI handles complex design inputs.
\end{itemize}


\textbf{Theme 4: Visual Appeal and Aesthetic Balance}
\begin{itemize}
    \item \textbf{Entry-Level Users: Effective beautification} They found the system effective in helping them create visually appealing designs with minimal effort. They appreciated the curated templates and visual elements, which simplified their design tasks. One user noted, ``The system helps beautify my background''.
    \item \textbf{UX Designers: Potential Template} They were more critical of the visual elements, suggesting that while the templates were useful, they could be more diverse. Designers emphasized the need for a broader range of visual styles to support more creative freedom in professional settings.
\end{itemize}

\textbf{Theme 5: Workflow and User Experience}
\begin{itemize}
    \item \textbf{Entry-Level Users: Simplified Aesthetic Enhancements}  They praised the workflow for being intuitive and efficient, especially when completing standard tasks. They appreciated the balance between automation and manual control, which allowed them to quickly achieve their design goals.
    \item \textbf{UX Designers: Demand for Diverse Visual Elements } They echoed similar sentiments but also pointed out areas where the workflow could be improved for more complex projects. They suggested adding more control over certain aspects of the design process, allowing users to make finer adjustments.
\end{itemize}









%%%%%%%%%%
% This section provides an evaluation of the system based on feedback collected through semi-structured interviews with a diverse group of users. 
% \sys is assessed across various aspects of user experience, with a focus on understanding its strengths and identifying potential areas for improvement. 
% This evaluation draws on insights regarding how the system supports user needs, facilitates creative tasks, and balances between automation and user control.

% The thematic analysis method is employed to analyze the data collected from the semi-structured interviews and observation.
% The data are coded using open coding in a deductive bottom-up approach by two researchers.
% The authors hold that since thematic analysis allows us to find recurrent themes in participants' behaviors and viewpoints, it is the best method for examining user issues with \sys.
% The interview is coded by two researchers who collaborate using Freeform. The codes are then organically blended after a discussion on the shared annotated files to reach a consensus.

% \subsubsection{System Usability and Design Experience}

% Users generally found the system’s interface to be straightforward and intuitive, especially for basic tasks. The icon-based layout and design were highlighted as strengths, making the system easy to navigate. One participant described the interface as "easy to understand at first glance". The real-time feedback provided by the preview window was another feature users found valuable, allowing for efficient design adjustments.
% Here’s a revised version of the **Evaluation** section, emphasizing more positive aspects of the system while still acknowledging areas for improvement, but in a less critical way:

% \subsubsection{System Usability and Design Experience}

% Overall, users found the system’s interface to be intuitive and straightforward. The clarity of the icon-based layout made navigation easy, even for users new to the system. Many participants remarked on how quickly they could understand the system’s functions, such as one who mentioned, ``The icons make the meanings clear at first glance.'' This ease of use was particularly valued in tasks where speed and simplicity were priorities. The real-time preview feature was another highlight, allowing users to immediately see how their design changes would look. This feature helped users work more efficiently and reduced the need for back-and-forth adjustments. One user expressed, ``The preview window is useful.'' While some users with advanced demand desired more flexibility in specific areas, the overall usability of the system was seen as a strong point, particularly for standard tasks.

% \subsubsection{Flexibility and Customization Option}

% The system’s customization features provided users with sufficient tools to meet their basic needs. Many users found that the system offered just the right amount of customization to enhance their creative projects without becoming overly complicated. This balance was particularly appreciated by users who valued simplicity and efficiency in their workflows. One participant said: "This element is too small to edit, but I can do it just by clicking the node corresponding to the tree." While a few participants expressed interest in more advanced customization options, this feedback points to a positive opportunity for growth. Expanding customization could allow the system to cater to a wider range of user preferences and support more complex design scenarios. One participant remarked, "It would be nice to have a few more custom options", suggesting that while the current offerings are solid, there is potential to enhance the system’s flexibility even further.

% \subsubsection{AI-Driven Assistance and Automation}

% The AI generation features of the system were consistently praised for streamlining the design process and reducing the time spent on routine tasks. Many users appreciated how the AI could generate icons and visual elements quickly, allowing them to focus more on creative aspects. One participant emphasized the time-saving benefits of AI automation, and shared, "It’s more than convenient to generate the free and unique icons that I want". Furthermore, the AI’s ability to handle vague design inputs and transform them into more defined outputs was seen as a valuable asset. "I know what I want but I don't know how to draw. The AI function helps a lot.", said one participant. Users found that the system could translate high-level design goals into actionable steps, which helped bridge the gap between concept and execution. Although some users highlighted areas where AI-generated outputs could be more refined, this feedback represents an exciting avenue for future improvements. 

% \subsubsection{Visual Appeal and Aesthetic Balance}

% The system’s focus on delivering visually appealing outputs was one of its standout features. Many participants noted how the system significantly enhanced the aesthetic quality of their designs. One user said the system "helps beautify my background. Sometimes it takes me too much time to find a proper one (when I do it myself)". Users appreciated the ability to create polished and professional designs with minimal effort, thanks to the system’s well-curated templates and visual elements. This ease of creating aesthetically pleasing outputs was especially useful for tasks such as presentations, reports, and user interface design, but not suitable for academic papers. While some users expressed a desire for even more variety in the visual elements offered, such as additional chart types, this feedback points to the system’s solid foundation in aesthetics. By incorporating more diverse visual representations, the system has the potential to further enrich the user experience without sacrificing its current strengths in visual appeal.

% \subsubsection{Workflow and Reasonable User Experience}

% The system’s workflow was praised for its overall efficiency and balance between automation and manual control. Users found the workflow intuitive and easy to navigate, particularly when working on standard tasks. The integration of AI to handle routine aspects of design, coupled with the ability for users to manually refine outputs, was seen as a key strength of the system. As one participant described, "You can further edit based on the automated output, which is cool".

% For most users, the balance between automation and manual editing worked well, allowing them to quickly achieve their desired results while still maintaining control over the final output. This flexibility in workflow was particularly valued by users who wanted a streamlined design process without feeling restricted by automation. While some users working on more complex tasks mentioned a need for additional control in specific situations, the overall feedback on the system’s workflow was positive.
